NCP: Neural Correspondence Prior for Effective Unsupervised Shape Matching

We present Neural Correspondence Prior (NCP), a new paradigm for computing correspondences between 3D shapes. Our approach is fully unsupervised and can lead to high-quality correspondences even in challenging cases such as sparse point clouds or non-isometric meshes, where current methods fail. Our first key observation is that, in line with neural priors observed in other domains, recent network architectures on 3D data, even without training, tend to produce pointwise features that induce plausible maps between rigid or non-rigid shapes. Secondly, we show that given a noisy map as input, training a feature extraction network with the input map as supervision tends to remove artifacts from the input and can act as a powerful correspondence denoising mechanism, both between individual pairs and within a collection. With these observations in hand, we propose a two-stage unsupervised paradigm for shape matching by (i) performing unsupervised training by adapting an existing approach to obtain an initial set of noisy matches, and (ii) using these matches to train a network in a supervised manner. We demonstrate that this approach significantly improves the accuracy of the maps, especially when trained within a collection. We show that NCP is data-efficient, fast, and achieves state-of-the-art results on many tasks. Our code can be found online: https://github.com/pvnieo/NCP.

==> body/3.0.background.tex <==
\section*{Background \& Notation}

Our work uses the functional map framework as a first estimator for p2p maps, and feature learning to learn robust features that allow extracting good correspondences using the nearest neighbor. We provide a brief overview in the next section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Background on Functional Map and Feature Learning}

\paragraph{Functional Maps}
As we will see in \cref{sec:non-rigid-corr}, the functional map (fmap) framework will be used for the first stage of our algorithm. For this, we follow the general strategy of recent fmap-based techniques \cite{donati2020deep,attaiki2021dpfm,sharma2020weakly,roufosse2019unsupervised,sharp2021diffusion}, as follows: given source and target shapes $\mathcal{M}$ and $\mathcal{N}$, represented as either triangular meshes or point clouds, having $m$ and $n$ vertices respectively, we pre-compute their Laplace-Beltrami operator, and store their first $k$ eigenfunctions in the matrices $\Phi_{\mathcal{M}} \in \mathbb{R}^{m \times k}$ and $\Phi_{\mathcal{N}} \in \mathbb{R}^{n \times k}$ respectively. Using a Siamese network $\mathcal{F}_{\theta}$, we compute for each shape a $d$-dimensional descriptor $\mathcal{F}_{\theta}(\mathcal{M}) = \mathbf{F} \in \mathbb{R}^{m \times d}$ and $\mathcal{F}_{\theta}(\mathcal{N}) = \mathbf{G} \in \mathbb{R}^{n \times d}$ respectively. These descriptors are then projected to the spectral domain to form the spectral features $\mathbf{A} = \Phi_{\mathcal{M}}^{\dagger} \mathbf{F}$ and $\mathbf{B} = \Phi_{\mathcal{N}}^{\dagger} \mathbf{G}$. A functional map is then computed by solving the following linear system:

\begin{align}
\label{eq:fmap_energy}
C_{opt} = \argmin_{C} \| C\mathbf{A} - \mathbf{B} \| + \lambda \|C \Delta_{\mathcal{M}} - \Delta_{\mathcal{N}} C \|.
\end{align}

where $\Delta_{\mathcal{M}},\Delta_{\mathcal{N}}$ are diagonal matrices of Laplace-Beltrami eigenvalues of the corresponding shapes and $\lambda$ is a scalar hyper-parameter.

Following the unsupervised literature \cite{roufosse2019unsupervised,sharma2020weakly,sharp2021diffusion}, the Siamese network $\mathcal{F}_{\theta}$ is trained by imposing structural properties on the fmap $C$ such as bijectivity and orthogonality. In fact, given the fmap $C_{\mathcal{M}\mathcal{N}}$ from $\mathcal{M}$ to $\mathcal{N}$, and $C_{\mathcal{N}\mathcal{M}}$ from $\mathcal{N}$ to $\mathcal{M}$, the bijectivity constraint is such that $C_{\mathcal{M}\mathcal{N}}C_{\mathcal{N}\mathcal{M}} = \mathbb{I}_k$, and the orthogonality constraint requires that $C_{\mathcal{M}\mathcal{N}}^{\top} C_{\mathcal{M}\mathcal{N}} = \mathbb{I}_k$. $\mathbb{I}_k$ denotes the identity matrix of size $k$ and $\bullet^{\top}$ is the matrix transpose operator.


\paragraph{Feature Learning}

The goal of feature learning is to learn robust descriptors that can allow direct nearest-neighbor matching in the descriptor space. In this work, we will use the contrastive loss PointInfoNCE \cite{xie2020pointcontrast}, i.e., given a set of matched points $\mathcal{P}$, and two features of dimension $d$, it is formulated as follows:

\begin{align}
	&\mathcal{L}_{\text{NCE}} = - \sum_{(i,j) \in \mathcal{P}} \log \dfrac{\exp( d(\mathbf{F}_i , \mathbf{G}_j) / \tau)}{\sum_{(\cdot, k) \in \mathcal{P}} \exp( d(\mathbf{F}_i , \mathbf{G}_k) / \tau)}
	\label{eq:PointInfoNCELoss}
\end{align}

where $\tau$ is a temperature parameter, and $d(\cdot,\cdot)$ is the Euclidean distance between the two features. The purpose of this loss is to force the distance between the features of the matched points to be minimized, while this distance must be maximized between the unmatched points. The NCE loss is applied to each point individually and thus cannot penalize the consistency of the matches at all. To remedy this, the LIE loss \cite{Marin2020CorrespondenceLV} is used. Given the extracted features $\mathbf{F}$ and $\mathbf{G}$, and the coordinate \textit{xyz} of the shape $\mathcal{M}$ represented by the matrix $\mathbf{M} \in \mathbb{R}^{m \times 3}$, we first compute the soft correspondences matrix $S_{\mathcal{M}\mathcal{N}}$ and then formulate the LIE loss as follows

\begin{align}
	&\mathcal{L}_{\text{LIE}} = \lVert S_{\mathcal{M}\mathcal{N}} \mathbf{M} -  \Pi_{\mathcal{M}\mathcal{N}}^{gt} \mathbf{M}\rVert_2^2,
	\label{eq:LIELoss}\\
	&(S_{\mathcal{M}\mathcal{N}})_{ij} = \frac{\exp(- \lVert \mathbf{F}_i - \mathbf{G}_j \rVert_2)}{\sum_{k=1}^{n} \exp(- \lVert \mathbf{F}_i - \mathbf{G}_k \rVert_2}
\end{align}

where $\Pi_{\mathcal{M}\mathcal{N}}^{gt}$ is the ground truth p2p correspondence matrix.

==> body/99.checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}




\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See \cref{sec:conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See supplementary}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See supplementary}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See supplementary}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Our code can be found online: \url{https://github.com/pvnieo/NCP}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See \cref{sec:application} and Supp Mat}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{In some experiments when it's not prohibitively expensive}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Supplementary}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{The used datasets are publicly available.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}
